SuperQuadricOcc: Real-Time Self-Supervised Semantic Occupancy Estimation with Superquadric Volume Rendering

Self-supervision for semantic occupancy estimation is appealing as it removes the labour-intensive manual annotation, thus allowing one to scale to larger autonomous driving datasets. Superquadrics offer an expressive shape family very suitable for this task, yet their deployment in a self-supervised setting has been hindered by the lack of efficient rendering methods to bridge the 3D scene representation with 2D training pseudo-labels. To address this, we introduce SuperQuadricOcc, the first self-supervised occupancy model to leverage superquadrics for scene representation. To overcome the rendering limitation, we propose a real-time volume renderer that preserves the fidelity of the superquadric shape during rendering. It relies on spatial superquadric-voxel indexing, restricting each ray sample to query only nearby superquadrics, thereby greatly reducing memory usage and computational cost. Using drastically fewer primitives than prior Gaussian-based methods, SuperQuadricOcc achieves state-of-the-art RayIoU on Occ3D-nuScenes with real-time inference and a substantially reduced memory footprint, while also outperforming Gaussian-based baselines on downstream occupancy forecasting and trajectory estimation.

==> tab/supplementary_material/ablation_main.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.05}
\caption{\textbf{SuperQuadricOcc-Render ablation studies} on Occ3D-nuScenes \cite{tian2023occ3d} and OpenOccv2 \cite{tong2023scene} datasets. The grey row is the preferred setting. Lat. denotes rendering latency in milliseconds.}

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}c@{\hspace{0.35em}}c@{\hspace{0.35em}}c@{\hspace{0.35em}}c@{}}

\begin{tabular}{c|cc|cc|c}
\toprule
\multirow{2}{*}{$\mathcal{N}$}
& \multirow{2}{*}{\textbf{IoU}}
& \multirow{2}{*}{\textbf{mIoU}}
& \multicolumn{2}{c|}{\textbf{RayIoU}}
& \multirow{2}{*}{\textbf{Lat.}} \\
&
&
& \textbf{Occ3D} & \textbf{OpenOccv2}
& \\
\midrule
3 & 38.86 & 14.53 & 14.19 & 15.23 & \textbf{13.54} \\
\rowcolor{black!5}
5 & \textbf{41.10} & 15.80 & 17.21 & 17.87 & 17.18 \\
\rowcolor{white}
7 & 40.65 & \textbf{15.88} & \textbf{18.06} & \textbf{18.43} & 29.73 \\
\bottomrule
\end{tabular}

&

\begin{tabular}{c|cc|cc|c}
\toprule
\multirow{2}{*}{$\kappa$}
& \multirow{2}{*}{\textbf{IoU}}
& \multirow{2}{*}{\textbf{mIoU}}
& \multicolumn{2}{c|}{\textbf{RayIoU}}
& \multirow{2}{*}{\textbf{Lat.}} \\
&
&
& \textbf{Occ3D} & \textbf{OpenOccv2}
& \\
\midrule
$1e^{-2}$ & 39.45 & 15.24 & 16.68 & 17.42 & \textbf{15.36} \\
$1e^{-4}$ & \textbf{41.15} & 15.69 & \textbf{17.44} & \textbf{18.05} & 16.86 \\
\rowcolor{black!5}
None & 41.10 & \textbf{15.80} & 17.21 & 17.87 & 17.18 \\
\bottomrule
\end{tabular}

&

\begin{tabular}{c|cc|cc|c}
\toprule
\multirow{2}{*}{$N$}
& \multirow{2}{*}{\textbf{IoU}}
& \multirow{2}{*}{\textbf{mIoU}}
& \multicolumn{2}{c|}{\textbf{RayIoU}}
& \multirow{2}{*}{\textbf{Lat.}} \\
&
&
& \textbf{Occ3D} & \textbf{OpenOccv2}
& \\
\midrule
1,200  & 39.69 & 14.96 & 16.28 & 16.99 & \textbf{16.33} \\
\rowcolor{black!5}
1,600  & 41.10 & 15.80 & 17.21 & 17.87 & 17.18 \\
\rowcolor{white}
2,000  & 41.36 & \textbf{16.08} & \textbf{17.71} & \textbf{18.25} & 20.16 \\
4,000  & 40.24 & 15.92 & 17.51 & 17.99 & 34.84 \\
10,000 & \textbf{42.00} & 15.86 & 16.38 & 17.03 & 91.18 \\
\bottomrule
\end{tabular}

&

\begin{tabular}{c|cc|cc|c}
\toprule
\multirow{2}{*}{$L$}
& \multirow{2}{*}{\textbf{IoU}}
& \multirow{2}{*}{\textbf{mIoU}}
& \multicolumn{2}{c|}{\textbf{RayIoU}}
& \multirow{2}{*}{\textbf{Lat.}} \\
&
&
& \textbf{Occ3D} & \textbf{OpenOccv2}
& \\
\midrule
50  & 40.61 & 15.64 & 17.30 & 17.85 & \textbf{12.68} \\
75  & 40.89 & 15.49 & 16.90 & 17.65 & 15.30 \\
\rowcolor{black!5}
100 & 41.10 & 15.80 & 17.21 & 17.87 & 17.18 \\
\rowcolor{white}
125 & 41.14 & 15.83 & 17.14 & 17.87 & 19.77 \\
150 & \textbf{41.53} & \textbf{15.85} & \textbf{17.52} & \textbf{18.06} & 21.12 \\
\bottomrule
\end{tabular}

\end{tabular}
\end{adjustbox}

\label{tab:main_abl}
\end{table*}

==> tab/supplementary_material/benchmark.tex <==
\begin{table}[htpb]
\caption{\textbf{Render Benchmark:} Render time for 10,000 SuperQuadrics, $512\times1408$ resolution, and max scene resolution. Max scene resolution refers to voxel resolution of $400\times400\times32$ for voxel-based methods, and/or ray samples $L=200$ for volume render methods. The best result overall is highlighted in \textbf{bold}.} 
\centering 
\begin{adjustbox}{width=0.40\linewidth}
\begin{tabular}{l|cc}
    \toprule
    \textbf{Model} & \textbf{Latency} & \textbf{Memory} \\
    \midrule
    MLGA & - \\
    Gaussianization & - \\
    Voxel NeRF & - \\
    SQOcc-R & - \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:benchmark}
\end{table}

==> tab/supplementary_material/depth_80m.tex <==
\begin{table}[htpb]
\caption{\textbf{Depth Estimation performance on nuScenes} For 80m range.}
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l|cc|cc|ccc}
    \toprule
    & \textbf{Abs}
    & \textbf{Sq}
    & \multicolumn{2}{c|}{\textbf{RMSE} }
    %& \textbf{RMSE}
    & \multicolumn{3}{c}{$\boldsymbol{\delta}$}
    % & $\boldsymbol{\delta\!<\!1.25} \uparrow$
    % & $\boldsymbol{\delta\!<\!1.25^2} \uparrow$
    % & $\boldsymbol{\delta\!<\!1.25^3} \uparrow$
    \\
    \multirow{-2}{*}{\textbf{Method}}
    & \textbf{Rel} $\downarrow$
    & \textbf{Rel} $\downarrow$
    & $\downarrow$
    & \textbf{log} $\downarrow$
    & $\boldsymbol{<\!\!1.25} \uparrow$
    & $\boldsymbol{<\!\!1.25^2} \uparrow$
    & $\boldsymbol{<\!\!1.25^3} \uparrow$ \\
    \midrule
    MLGA &
    0.194 & 1.934 & 8.236 & 0.569 & 0.714 & 0.854 & 0.914 \\
    Gaussianisation &
    0.203 & 1.880 & \textbf{8.071} & \textbf{0.351} & 0.711 & 0.852 & 0.919 \\
    Voxel NeRF & 
    0.208 & 2.023 & 8.383 & 0.387 & 0.683 & 0.822 & 0.894 \\
    \renderShort{} (Ours) &
    \textbf{0.190} & \textbf{1.825} & 8.163 & 0.353 & \textbf{0.717} & \textbf{0.857} & \textbf{0.920} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:80m_depth}
\end{table}


==> tab/supplementary_material/rayIoU_class.tex <==
\begin{table*}[htp]
    \caption{\textbf{SuperQuadricOcc render method RayIoU comparison per class on Occ3D-nuScenes \cite{tian2023occ3d}:} All models are self-supervised. Classwise metrics are taken from RayIoU@2. The best-performer is highlighted in \textbf{bold}.}
     %\andreic{Are mem. and fps identical for SuperQuadricOcc and SQ-Nerf identical?}
  \centering
  \setlength{\tabcolsep}{3pt}
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{
    @{}l
    | >{\columncolor{blue!5}}c
    |  >{\columncolor{blue!5}}c
        >{\columncolor{blue!5}}c
        >{\columncolor{blue!5}}c
    |*{15}{c}
    @{}
}
    \toprule
\textbf{Model} 
& \rotatebox{\myangle}{\textbf{RayIoU}}
& \rotatebox{\myangle}{\textbf{RayIoU@1}}
& \rotatebox{\myangle}{\textbf{RayIoU@2}}
& \rotatebox{\myangle}{\textbf{RayIoU@4}}
& \rotatebox{\myangle}{\textcolor{barrier}{$\blacksquare$} barrier} & \rotatebox{\myangle}{\textcolor{bicycle}{$\blacksquare$} bicycle} & \rotatebox{\myangle}{\textcolor{bus}{$\blacksquare$} bus} & \rotatebox{\myangle}{\textcolor{car}{$\blacksquare$} car} & \rotatebox{\myangle}{\textcolor{construction}{$\blacksquare$} const. veh.} & \rotatebox{\myangle}{\textcolor{motorcycle}{$\blacksquare$} motorcycle} & \rotatebox{\myangle}{\textcolor{pedestrian}{$\blacksquare$} pedestrian} & \rotatebox{\myangle}{\textcolor{cone}{$\blacksquare$} traffic cone} & \rotatebox{\myangle}{\textcolor{trailer}{$\blacksquare$} trailer} & \rotatebox{\myangle}{\textcolor{truck}{$\blacksquare$} truck} & \rotatebox{\myangle}{\textcolor{driveable}{$\blacksquare$} drive. surf.} & \rotatebox{\myangle}{\textcolor{sidewalk}{$\blacksquare$} sidewalk} & \rotatebox{\myangle}{\textcolor{terrain}{$\blacksquare$} terrain} & \rotatebox{\myangle}{\textcolor{manmade}{$\blacksquare$} manmade} & \rotatebox{\myangle}{\textcolor{vegetation}{$\blacksquare$} vegetation} \\
    \midrule 
   MLGA & 12.1 & 7.3 & 11.9 & 17.2 & 8.4 & 6.0 & 31.2 & 23.6 & 3.9 & 5.5 & 9.6 & 4.8 & \textbf{1.2} & 24.3 & 20.2 & 5.0 & 6.0 & 16.4 & 15.9
    \\
    Gaussianisation & 16.4 & 10.6 & 16.2 & 22.3 & 12.0 & 7.1 & 25.9 & 20.2 & \textbf{5.0} & 6.7 & 15.1 & 12.8 & 0.2 & 24.4 & 42.8 & 12.9 & 14.5 & 22.6 & 23.5
    \\
    Voxel NeRF & 18.8 & 13.0 & 18.8 & 24.5 & \textbf{16.3} & 7.0 & 35.1 & 29.5 & 2.7 & 7.2 & 17.2 & \textbf{16.1} & 0.0 & 28.5 & \textbf{47.0} & \textbf{15.2} & \textbf{15.2} & 23.3 & 21.4
    \\
    SQOcc-R (Ours) & \textbf{19.6} & \textbf{13.5} & \textbf{19.6} & \textbf{25.6} & 14.3 & \textbf{8.8} & \textbf{38.0} & \textbf{31.2} & 4.9 & \textbf{8.6} & \textbf{18.1} & 15.1 & 0.3 & \textbf{30.7} & 45.9 & 14.3 & \textbf{15.2} & \textbf{24.1} & \textbf{23.9}
    \\
    %GaussianFlowOcc & - & - & - & - & 12.60 & 7.20 & 39.80 & 30.70 & 5.50 & 11.20 & 16.50 & 13.70 & 0.10 & 28.70 & 35.40 & 13.30 & 14.40 & 23.70 & 22.30 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:rayiou_class}
\end{table*}



% \begin{table*}[t]
%     \caption{\textbf{State-of-the-art model comparison on Occ3D-nuScenes \cite{tian2023occ3d}:} Rep. denotes the method of scene representation: Gauss - Gaussian; Quad - SuperQuadric. Mem. denotes the maximum memory (GB) during inference (rendering pipeline not included). All models are self-supervised. The best-performer is highlighted in \textbf{bold}.}
%      %\andreic{Are mem. and fps identical for SuperQuadricOcc and SQ-Nerf identical?}
%   \centering
%   \setlength{\tabcolsep}{3pt}
%   \begin{adjustbox}{width=\textwidth}
%   \begin{tabular}{
%     @{}l
%     |>{\columncolor{red!5}}c
%     |>{\columncolor{green!5}}c
%         >{\columncolor{green!5}}c
%     | >{\columncolor{blue!5}}c
%         >{\columncolor{blue!5}}c
%     |*{15}{c}
%     @{}
% }
%     \toprule
% \textbf{Model} & \textbf{Rep.} & \textbf{Mem.} & \textbf{FPS} & \textbf{IoU} & \textbf{mIoU} & \rotatebox{\myangle}{\textcolor{barrier}{$\blacksquare$} barrier} & \rotatebox{\myangle}{\textcolor{bicycle}{$\blacksquare$} bicycle} & \rotatebox{\myangle}{\textcolor{bus}{$\blacksquare$} bus} & \rotatebox{\myangle}{\textcolor{car}{$\blacksquare$} car} & \rotatebox{\myangle}{\textcolor{construction}{$\blacksquare$} const. veh.} & \rotatebox{\myangle}{\textcolor{motorcycle}{$\blacksquare$} motorcycle} & \rotatebox{\myangle}{\textcolor{pedestrian}{$\blacksquare$} pedestrian} & \rotatebox{\myangle}{\textcolor{cone}{$\blacksquare$} traffic cone} & \rotatebox{\myangle}{\textcolor{trailer}{$\blacksquare$} trailer} & \rotatebox{\myangle}{\textcolor{truck}{$\blacksquare$} truck} & \rotatebox{\myangle}{\textcolor{driveable}{$\blacksquare$} drive. surf.} & \rotatebox{\myangle}{\textcolor{sidewalk}{$\blacksquare$} sidewalk} & \rotatebox{\myangle}{\textcolor{terrain}{$\blacksquare$} terrain} & \rotatebox{\myangle}{\textcolor{manmade}{$\blacksquare$} manmade} & \rotatebox{\myangle}{\textcolor{vegetation}{$\blacksquare$} vegetation} \\
%     \midrule 
%     DistillNeRF \cite{wang2024distillnerf} & Voxel & - & 2.8 & 29.1 & 10.1 & 1.4 & 2.1 & 10.2 & 10.1 & 2.6 & 2.0 & 5.5 & 4.6 & 1.4 & 7.9 & 43.0 & 16.9 & 15.0 & 14.1 & 15.1 \\
%     SelfOcc \cite{huang2024selfocc} & Voxel & 3.00 & 7.4 & 45.0 & 10.5 & 0.2 & 0.7 & 5.5 & 12.5 & 0.0 & 0.8 & 2.1 & 0.0 & 0.0 & 8.3 & 55.5 & 26.3 & 26.5 & 14.2 & 5.6 \\
%     OccNeRF \cite{zhang2023occnerf} & Voxel & 12.68 & 5.4 & \textbf{46.4} & 10.8 & 0.8 & 0.8 & 5.1 & 12.5 & 3.5 & 0.2 & 3.1 & 1.8 & 0.5 & 3.9 & 52.6 & 20.8 & 24.8 & 18.5 & 13.2 \\
%     GaussianOcc \cite{gaussianocc} & Voxel & 11.81 & 5.4 & 42.9 & 11.3 & 1.8 & 5.8 & 14.6 & 13.6 & 1.3 & 2.8 & 8.0 & 9.8 & 0.6 & 9.6 & 44.6 & 20.1 & 17.6 & 8.6 & 10.3 \\
%     %SuperQuadricOcc \cite{hayes2025superquadricocc} & Quad & \textbf{0.70} & \textbf{21.5} & 33.67 & 12.69 & 5.78 & 5.69 & 16.32 & 13.06 & 3.72 & 5.69 & 3.94 & 3.54 & 2.56 & 11.94 & 43.58 & 20.66 & 24.15 & 14.45 & 15.29 \\
%     GaussTR \cite{jiang2025gausstr} & Gauss & 1.97 & 0.3 & 44.5 & 13.8 & 6.5 & 8.5 & \textbf{21.8} & \textbf{24.3} & 6.3 & \textbf{15.5} & 7.9 & 1.9 & \textbf{6.1} & \textbf{17.2} & 37.0 & 17.2 & 7.2 & \textbf{21.2} & 10.0 \\
%     EasyOcc \cite{hayes2025easyocc} & Voxel & - & 5.4 & 38.9 & 15.7 & 1.9 & 6.7 & \textbf{15.1} & 21.7 & 2.7 & 8.1 & 15.3 & 11.1 & 1.4 & 12.8 & 55.8 & 27.9 & 22.1 & 16.1 & 17.3 \\
%     %\midrule
%     GaussianFlowOcc \cite{boeder2025gaussianflowocc} & Gauss & 2.85 & 9.6 & 40.5 & 16.7 & 6.7 & 9.2 & 17.5 & 16.5 & 4.0 & 11.9 & 8.8 & 9.7 & 0.6 & 12.3 & 49.3 & 30.8 & \textbf{34.6} & 17.4 & 20.8 
%     \\
%     TT-Occ \cite{zhang2025tt} & Gauss & 9.90 & 0.7 & - & 16.7 & \textbf{21.5} & \textbf{10.5} & 10.7 & 14.7 & \textbf{11.9} & 12.3 & 9.7 & \textbf{12.2} & 4.4 & 7.9 & 48.3 & 23.7 & 28.3 & 14.1 & 20.2 \\
%     \midrule
%     SuperQuadricOcc (Ours) & Quad & \textbf{0.70} & \textbf{21.5} & 43.5 & \textbf{17.1} & 7.0 & 8.3 & 16.6 & 14.8 & 3.4 & 9.1 & 8.0 & 8.8 & 1.1 & 12.0 & \textbf{64.7} & \textbf{31.4} & 34.3 & 16.6 & \textbf{21.0}
%     \\
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
%   \label{tab:sota_occ3d}
% \end{table*}
